The Maximum Binary Tree Problem

We introduce and investigate the approximability of the maximum binary tree problem (MBT) in directed and undirected graphs. The goal in MBT is to find a maximum-sized binary tree in a given graph. MBT is a natural variant of the well-studied longest path problem, since both can be viewed as finding a maximum-sized tree of bounded degree in a given graph. The connection to longest path motivates the study of MBT in directed acyclic graphs (DAGs), since the longest path problem is solvable efficiently in DAGs. In contrast, we show that MBT in DAGs is in fact hard: it has no efficient $\exp(-O(\log n/ \log \log n))$-approximation algorithm under the exponential time hypothesis, where $n$ is the number of vertices in the input graph. In undirected graphs, we show that MBT has no efficient $\exp(-O(\log^{0.63}{n}))$-approximation under the exponential time hypothesis. Our inapproximability results rely on self-improving reductions and structural properties of binary trees. We also show constant-factor inapproximability assuming $\text{P}\neq \text{NP}$. In addition to inapproximability results, we present algorithmic results along two different flavors: (1) We design a randomized algorithm to verify if a given directed graph on $n$ vertices contains a binary tree of size $k$ in $2^k \text{poly}(n)$ time. (2) Motivated by the longest heapable subsequence problem, introduced by Byers, Heeringa, Mitzenmacher, and Zervas (ANALCO 2011), which is equivalent to MBT in permutation DAGs, we design efficient algorithms for MBT in bipartite permutation graphs.

==> bdd_tw.tex <==
\section{An efficient algorithm for finding a maximum binary tree in bounded treewidth graphs}\label{sec:boundedtreewidth}

In this section, we prove Theorem~\ref{theorem:bounded-treewidth} by designing an efficient dynamic programming algorithm to find a maximum binary tree in graphs with bounded treewidth. We will focus on the rooted version of the problem as defined below. 

\begin{problem}{\rumaxBT}
	Given: An undirected graph $G$ and a root $s \in V(G)$.
	
	Goal: A binary tree in $G$ containing $s$ where $\deg_T(s) \leq 2$ with maximum number of vertices.
\end{problem}

Now we introduce the definition of \emph{treewidth}.

\begin{definition} \label{def:tree-decomposition}
A {\em tree decomposition} of an undirected graph $G$ is given by $\cT = (T,\{X_t\}_{t \in V(T)})$, where $T$ is a tree in which every tree node $i \in V(T)$ is assigned a subset $X_i \subseteq V(G)$ of vertices of $G$, called a bag, such that the following conditions are satisfied:
\begin{enumerate} [label=(T\arabic*)]
\item \label{T1} $\cup_{i \in V(T)} X_i = V(G)$.
\item \label{T2} For each $\{u,v\} \in E(G)$, there is a tree node $i \in V(T)$ in the tree $T$ such that both $u$ and $v$ are in $X_i$.
\item \label{T3} For each vertex $u \in V(G)$, if there exist two tree nodes $i, j\in V(T)$ in the tree $T$ such that $u$ is in both $X_i$ and $X_j$, then $u\in X_k$ for every tree node $k \in V(T)$ on the unique path between $i$ and $j$.
\end{enumerate}
For ease of distinction, we will denote $i \in V(T)$ as a \emph{tree node} and the set $X_i$ as a \emph{bag} of the tree decomposition $\cal T$. The \emph{width} of a tree decomposition is $\max_{i \in V(T)}\{|X_i|-1\}$. The \emph{treewidth} $w_G$ of the graph $G$ is the minimum width among all possible tree decompositions. A tree decomposition with treewidth $w_G$ can be found in $(w_G 2^{w_G})^{O(w_G^2)}|V(G)|$ time \cite{bodlaender1996linear}.
\end{definition}

\subsection{Outline of the algorithm}
Our algorithm consists of two parts:
\begin{enumerate}
    \item Design a linear time algorithm to solve \rumaxBT.
    \item Reduce \umaxBT to \rumaxBT.
\end{enumerate}

For the first part, we will show the following theorem in the next sections.
\begin{restatable}{theorem}{rbddtw} \label{thm:rbddtw}
Let $s \in V(G)$ be a root. Given a tree decomposition of $G$ with width $w_G$, \rumaxBT can be solved in ${w_G}^{O(w_G)}|V(G)|$ time.
\end{restatable}

For the second part, by Theorem~\ref{thm:rbddtw}, given a tree decomposition of $G$ with width $w_G$, we can find a maximum binary tree of $G$ in $w_G^{O(w_G)}|V(G)|^2$ time by solving \rumaxBT for every possible choice of the root vertex in $G$. The time complexity can be brought down to linear as shown in the proof below. Corollary \ref{coro:bdd-MBT} proves Theorem \ref{theorem:bounded-treewidth}.

\begin{corollary}\label{coro:bdd-MBT}
Given a tree decomposition of $G$ with width $w_G$, \umaxBT can be solved in ${w_G}^{O(w_G)}|V(G)|$ time.
\end{corollary}

\begin{proof}
\umaxBT with $G$ as the input graph can be solved by the following reduction to \rumaxBT in a graph whose treewidth is one larger than the treewidth of $G$:
\begin{enumerate}
\item Construct $G'$ by adding a vertex $s$ and a binary tree $B$ such that:
\begin{enumerate}
\item $s$ is adjacent to all the vertices in $V(G)$,
\item $s$ is adjacent to the root of $B$, and
\item $|E(B)| = |E(G)|$.
\end{enumerate}
\item Solve \rumaxBT on $G'$ rooted at $s$ to obtain the maximum binary tree $T'$ of $G'$.
\item Let $v \in V(G)$ be the vertex such that $\{v,s\} \in E(T')$. Pick the subtree of $T'$ rooted at $v$.
\end{enumerate}
This is a generic reduction from \umaxBT to \rumaxBT (but not approximation-preserving). We note that the treewidth of the graph $G'$ is one larger than the treewidth of $G$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:rbddtw}}
We will prove Theorem \ref{thm:rbddtw} in this section. We begin with a convenient form of tree decompositions and associated notations in Section \ref{subsubsec:special-tree-decompositions}. We describe the subproblems of the dynamic program along with the recursive expressions for these subproblems and analyze the run-time in Section \ref{subsubsec:bddtw-dp}. We prove the correctness of the recursive expressions in Section \ref{sec:dp_pf}.

\subsubsection{Special tree decompositions} \label{subsubsec:special-tree-decompositions}
In this subsection, we will introduce a modified form of tree decomposition that will be convenient for our dynamic program. We also introduce the associated notations and prove a crucial edge disjointness property (Lemma \ref{lem:disjoint}). 

Given a tree decomposition $\cT$ with an arbitrarily chosen root, the parent-child and ancestor-descendant relationships between the tree nodes are defined naturally. With these relationships, it will be convenient to think of \emph{nice tree decompositions} (defined below) as rooted trees.

\begin{definition} \label{def:nice-tree-decomposition}
A {\em nice tree decomposition} of an undirected graph $G$ is a tree decomposition $\cT = (T,\{X_t\}_{t \in V(T)})$ where $T$ is rooted at a tree node $r \in V(T)$ such that:

\begin{enumerate}
\item $X_l = \emptyset$ for every leaf tree node $l \in V(T)$ and $X_r = \emptyset$.
\item Every non-leaf tree node $i$ is one of the following four types:
\begin{description}
\item[Introduce vertex:] Tree node $i$ has only one child $j$ with $X_i = X_j \cup \{v\}$ for some $v \in V(G) \setminus X_j$. In this scenario, we say that vertex $v$ is \emph{introduced} at tree node $i$.
\item[Drop:] Tree node $i$ has only one child $j$ with $X_i = X_j \setminus \{v\}$ for some $v \in X_j$. In this scenario, we say that vertex $v$ is \emph{dropped} at tree node $i$.
\item[Join:] Tree node $i$ has two children $j$ and $k$ with $X_i=X_j=X_k$.
\item[Introduce edge:] Tree node $i$ is labeled by an edge $\set{u,v} \in E(G)$ such that both $u$ and $v$ belong to $X_i$, and $i$ has only one child $j$ with $X_i = X_j$. In this scenario, we say that edge $\set{u,v}$ is \emph{introduced} at tree node $i$.
\end{description}
\item Every edge of $G$ is introduced at exactly one tree node.
\item Every edge $\{u,v\}$ is introduced at tree node $i$ which is between tree nodes $j$ and $k$ such that:
\begin{enumerate}
\item Node $j$ is an ancestor of node $k$.
\item Node $j$ either drops $u$ or drops $v$.
\item All tree nodes between node $j$ and node $k$ are of type introduce edge and they introduce edges incident at the vertex that $j$ drops.
\item Node $k$ is not of type introduce edge.
\end{enumerate}
\end{enumerate}
\end{definition}

Given a tree decomposition with width $w_G$, a nice tree decomposition with $O(w_G |V(G)|)$ tree nodes can be computed in $O(w_G^2 \max\{|V(G)|,|V(T)|\})$ time \cite{FPT-book}. We note that by \ref{T3}, each vertex in $V(G)$ is dropped \emph{only once}, but may be introduced several times in a nice tree decomposition.

In order to solve \rumaxBT, we construct $G^s$ from $G$ by adding a pendant vertex $s'$ and edge $\{s,s'\}$. Formally, $G^s:=(V(G) \cup \{s'\}, E(G) \cup \set{\set{s,s'}})$.

\begin{observation}
The maximum binary tree in $G$ rooted at $s$ can be obtained by finding a maximum binary tree in $G^s$ rooted at $s'$ and removing the vertex $s'$ and the edge $\{s,s'\}$ from the tree.
\end{observation}

Now we introduce a special tree decomposition of $G^s$.

\begin{definition}
Given a nice tree decomposition of $G$, an \emph{$s'$-special tree decomposition} of $G^s$ is a tree decomposition obtained by the following steps:
\begin{enumerate}
\item Obtain a nice tree decomposition of $G$ with width $w_G$.
\item Add $s'$ to each bag and insert a tree node that introduces the edge $\set{s,s'}$ between the tree node that drops $s$ and its child.
\end{enumerate}
\end{definition}

The idea behind this tree decomposition is to ensure that every bag contains the new root $s'$, which is useful in the definition of the subproblems for the dynamic program.

For brevity, we will denote the resulting $s'$-special tree decomposition of $G^s$ as $\cT  = (T,\{X_t\}_{t \in V(T)})$. Let $r$ be the root tree node of $T$. Since we will only care about the optimal structure that is stored locally with respect to a tree node, we will use the following notations.

\begin{definition}
For a tree node $i$, let 
\begin{enumerate}
\item $S_i$ denote the set of tree nodes consisting of all its descendants (including $i$),
\item $V_i := \bigcup_{j \in S_i}{X_j}$ be the {\em descendant vertices}, 
\item $E_i := \set{e\in E(G): e \text{ is introduced at some tree nodes in the subtree rooted at $i$}}$ be the {\em descendent edges}, and 
\item $G_i := (V_i, E_i)$.
\end{enumerate}
\end{definition}

With the above notations, we show a \emph{disjointness} property for the join tree nodes.
\begin{lemma} \label{lem:disjoint}
In an $s'$-special tree decomposition, suppose a join tree node $i$ has two children $j$ and $k$ with $X_i=X_j=X_k$. Then $(V_j \setminus X_i) \cap (V_k \setminus X_i) = \emptyset$ and $E_j \cap E_k = \emptyset$.
\end{lemma}

\begin{proof}
First, we show that $(V_j \setminus X_i) \cap (V_k \setminus X_i) = \emptyset$. Assume for the sake of contradiction that there is a vertex $v \in (V_j \setminus X_i) \cap (V_k \setminus X_i)$. Then there is a descendent tree node $d_j$ of $j$, such that $v \in X_{d_j} \setminus X_i$. Similarly, there is a descendent tree node $d_k$ of $k$, such that $v \in X_{d_k} \setminus X_i$. From \ref{T3}, the vertex $v$ must belong to the bag of every tree node that is on the unique path between tree nodes $d_j$ and $d_k$, and this includes tree node $i$. Hence, $v \in X_i$, a contradiction.

Next, we show that $E_j \cap E_k = \emptyset$. By Definition~\ref{def:nice-tree-decomposition}, a tree node that drops vertex $v$ is followed by descendant tree nodes that introduce edges with $v$ as an endvertex until a descendant tree node that is not of type introduce edge is reached. Therefore, the edge $\{u,v\}$ where $u \in X_i$ and $v \in X_i$ is not yet included in $E_i$. Consequently, any edge in $E_j$ cannot have both endvertices in $X_j = X_i$, i.e. it must have an endvertex in $V_j \setminus X_j=V_j\setminus X_i$. Similar argument implies that any edge in $E_k$ cannot have both endvertices in $X_k=X_i$, i.e., it must have an endvertex in $V_k\setminus X_k=V_k\setminus X_i$. From $(V_j \setminus X_i) \cap (V_k \setminus X_i) = \emptyset$, we must have $E_j \cap E_k = \emptyset$.
\end{proof}

\subsubsection{The dynamic program} \label{subsubsec:bddtw-dp}

Our algorithm solves subproblems in a bottom-up fashion beginning with the leaf tree nodes. For every tree node $i$ and for all possible $(X,\mathcal{P},D)$, where 
\begin{enumerate}
\item $X \subseteq X_i$, 
\item $\mathcal{P}$ is a partition $\{P_1, P_2, ..., P_q\}$ of $X$ with each part of $\mathcal{P}$ being non-empty, and 
\item $D:X \rightarrow \{0,1,2,3\}$ is a function specifying the degree constraints on the vertices of $X$,  
\end{enumerate}
let $\mbt_i(X,\cP,D)$ be the \emph{maximum number of edges} in a binary forest $F$ satisfying the following five constraints:

\begin{enumerate} [label=(DP\arabic*),align=left]
\item \label{DP1} $F$ is a subgraph of $G_i$,
\item \label{DP2} $s' \in X$,
\item \label{DP3} $X_i \cap V(F) = X$, i.e. the set of vertices in $F$ from $X_i$ is exactly $X$,
\item \label{DP4} $F$ has \emph{exactly} $q$ connected components (trees) $T_1, ..., T_q$ such that $ V(T_p) \cap X = P_p$ for each $p \in \{1,2,...,q\}$, i.e. each part of $\mathcal{P}$ corresponds to a single tree of $F$, and 
\item \label{DP5} $\deg_F(v) = D(v)$ for each $v \in X$, i.e. each vertex $v\in X$ has exactly $D(v)$ edges incident to it in $F$.
\end{enumerate}

A forest is \emph{feasible} for $\mbt_i(X,\cP,D)$ if it satisfies properties \ref{DP1}, \ref{DP2}, \ref{DP3}, \ref{DP4}, and \ref{DP5}. If a forest has the maximum number of edges among the feasible forests, then we say that this forest is \emph{optimal} for $\mbt_i(X,\cP,D)$. If there is no feasible forest for $\mbt_i(X,\mathcal{P},D)$, then we call the subproblem to be \emph{infeasible}. For example, $\mbt_i(X,\mathcal{P},D)$ where $D(v)=0$ for a vertex $v \in X \subseteq X_i$ in a part $P\in \mathcal{P}$ with $|P| \geq 2$ is infeasible. We will define $\mbt_i(X,\mathcal{P},D)=-\infty$ when the subproblem is infeasible.

We recall that $r$ is the root of the $s'$-special tree decomposition of $G^s$. The number of edges in the maximum binary tree of $G^s$ rooted at $s'$ is exactly $\mbt_r(X=\{s'\},\mathcal{P}=\set{\set{s'}},D(s')=1)$. We now provide the recurrence relations for the dynamic programming algorithm for each type of tree node.

\paragraph{Leaf:} Suppose $i$ is a leaf tree node. Then, 
\begin{equation*} \tag{DP-L} \label{eq:DP-L}
\mbt_i(X,\mathcal{P},D)=
\begin{cases}
0 &\text{if $X=\set{s'}, \cP=\set{\set{s'}}$, and $D(s')=0$,}\\
-\infty &\text{otherwise}.
\end{cases}
\end{equation*}
\paragraph{Introduce vertex:} Suppose $i$ introduces vertex $v$ and $j$ is the child of $i$ with $X_i=X_j\cup \{v\}$ for some $v\in V(G)\setminus X_j$. Consider the following conditions:
\begin{enumerate} [label=(IntroVertex \arabic*),align=left]
\item \label{IV1} $v\in X$ and either $\{v\}$ is not a part in $\cP$ or $D(v)>0$.
\item \label{IV2} $v \in X$, $\set{v}$ is a part in $\cP$, and $D(v)=0$.
\end{enumerate}
For $D:X\rightarrow \{0,1,2,3\}$, let $D':X\setminus \{v\}\rightarrow \{0,1,2,3\}$ be obtained by setting $D'(u)=D(u)$ for every $u\in X\setminus \{v\}$. Then, 
\begin{equation} \tag{DP-IV} \label{eq:DP-IV}
\mbt_i(X,\cP,D) =
\begin{cases}
-\infty & \text{if \ref{IV1},}\\
\mbt_j(X \setminus \set{v},\cP \setminus \set{\set{v}}, D') & \text{if \ref{IV2},}\\
\mbt_j(X,\cP,D) & \text{otherwise.}
\end{cases}
\end{equation}

\paragraph{Introduce edge:} Suppose $i$ introduces edge $\set{u,v}$ and $j$ is the child of $i$ with $X_i=X_j$. Consider the following condition:

\begin{enumerate} [label=(IntroEdge\arabic*),align=left]
\item \label{IE1} $u$ and $v$ are both in $X$ and in the same part $P\in \cP$.
\end{enumerate}

Suppose \ref{IE1} holds. Then let $\cP'$ be a partition of $X$ obtained from $\cP$ by splitting $P$ into two disjoint sets $P_u$ and $P_v$ such that $u \in P_u$ and $v \in P_v$, i.e. $\cP' = \cP \setminus \{P\} \cup \{P_u, P_v\}$, and $D':X\rightarrow \{0,1,2,3\}$ be obtained by setting $D'(w) = D(w)$ for $w \in X \setminus \set{u,v}$, $D'(u) = D(u)-1 \leq 3$, $D(u) \geq 1$, $D'(v) = D(v)-1 \leq 3$, and $D(v) \geq 1$. Then
\begin{equation} \tag{DP-IE} \label{eq:DP-IE}
\mbt_i(X,\cP,D) =
\begin{cases}
\max\{
\maxx_{\cP',D'}{\mbt_j(X,\cP',D')+1},
\mbt_j(X,\cP,D)\} & \text{if \ref{IE1},}\\
\mbt_j(X,\cP,D) & \text{otherwise.}
\end{cases}
\end{equation}

\paragraph{Drop:} Suppose $i$ drops vertex $v$ and $j$ is the child of $i$ with $X_i = X_j \setminus \{v\}$ for some $v \in X_j$. Let $\cP'$ be a partition obtained by adding $v$ to one of the existing parts of $\cP$ and $D':X\cup\set{v} \rightarrow \set{0,1,2,3}$ is obtained by setting $D'(u)=D(u)$ for $u \in X$ and $D'(v)$ is set to some value in $\{1,2,3\}$. Then
\begin{equation} \tag{DP-D} \label{eq:DP-D}
\mbt_i(X,\cP,D) = 
\max\left\{
\maxx_{\cP',D'}\left\{\mbt_j(X \cup \set{v},\cP',D')\right\},
\mbt_j(X,\cP,D)
\right\}.
\end{equation}

\paragraph{Join:}

Suppose $i$ has two children $j$ and $k$ with $X_i=X_j=X_k$. 

For arbitrary partitions $\cP^j, \cP^k$ of $X$, we obtain a graph $H(\cP^j,\cP^k)$ and a partition $\mathcal{Q}(\cP^j,\cP^k)$ as follows: for $b \in \{j,k\}$ we first construct an \emph{auxiliary graph} $H_b$ that contains vertices for every vertex in $X$ and vertices for every part in $\cP^b$, with the vertex corresponding to a part of $\cP^b$ being adjacent to all vertices that are in that part. We note that $V(H_j)\cap V(H_k)=X$ and $E(H_j)\cap E(H_k)=\emptyset$. We consider the \emph{merged graph} $H(\cP^j,\cP^k) := (V(H_j) \cup V(H_k), E(H_j) \cup E(H_k))$. Let $\mathcal{Q'}$ be a partition of $V(H(\cP^j,\cP^k))$ where vertices in the same connected component of $H$ belong to the same part of $\mathcal{Q'}$. Let $\mathcal{Q}(\cP^j, \cP^k)$ be the partition of $X$ obtained from $\mathcal{Q}'$ by restricting each part of $\mathcal{Q}'$ to elements in $X$. Namely, $\mathcal{Q}(\cP^j, \cP^k) = \{Q \cap X \mid Q \in \mathcal{Q'} \}$. We note that $\mathcal{Q}(\cP^j,\cP^k)$ can be found efficiently by running a depth first search on $H(\cP^j,\cP^k)$.

Let $(X,\cP,D)$ be the input at tree node $i$. Let $\cP^j$ and $\cP^k$ be partitions such that the graph $H(\cP^j,\cP^k)$ is a forest and the resulting partition $\mathcal{Q}(\cP^j,\cP^k)=\cP$. Let $D^j, D^k:X \rightarrow \set{0,1,2,3}$ be functions such that $D(v) = D^j(v)+D^k(v)$ for every $v \in X$. Then
\begin{equation} \tag{DP-J} \label{eq:DP-J}
\mbt_i(X,\cP,D) =
\begin{cases}
\maxx_{\cP^j,\cP^k,D^j,D^k}{\mbt_j(X,\cP^j,D^j)+\mbt_k(X,\cP^k,D^k),} \\
-\infty \text{ if there are no such $\cP^j,\cP^k,D^j$, and $D^k$.}
\end{cases}
\end{equation}

\paragraph{} When the root tree node $r$ is reached, the maximum number of edges of the binary tree in $G^s$ is $\mbt_r(X=\{s'\},P=\{\{s'\}\},D(s')=1)$. To find the optimal binary tree, we can simply backtrack through the subproblems to obtain an optimal solution.

This concludes the description of the algorithm. The proof of correctness is in Section~\ref{sec:dp_pf}. We proceed to analyze the running time. The bag of each tree node has at most $w_G+2$ vertices, so the number of subproblems per tree node is at most $(8w_G + 16)^{w_G + 2} = {w_G}^{O(w_G)}$, since for a tree node $i$ there are $2^{|X_i|}$ subsets $X \subseteq X_i$, at most $|X|^{|X|}$ partitions of $X$, and at most $4^{|X|}$ degree requirements. Solving a subproblem at a tree node requires considering at most all states from the children of that tree node, which takes $({w_G}^{O(w_G)})^2 = {w_G}^{O(w_G)}$ time. Thus, the running time for computing all the $\mbt$ values of a tree node is ${w_G}^{O(w_G)}$. We have thus proved Theorem~\ref{thm:rbddtw}.

\rbddtw*

\subsubsection{Correctness of the dynamic program} \label{sec:dp_pf}

We prove the correctness of the recursion expressions in the dynamic program described in the previous section.

\begin{lemma}
$\mbt_i(X,\cP,D)$ satisfies the recurrence relations given in \ref{eq:DP-L}, \ref{eq:DP-IV}, \ref{eq:DP-IE}, \ref{eq:DP-D}, and \ref{eq:DP-J}.
\end{lemma}
\begin{proof}
The proof consists of showing two parts: If $\mbt_i(X,\cP,D)$ is feasible, then the right hand side (RHS) of the recurrence formula should be the same as the left hand side (LHS), or equivalently, RHS is an upper bound and lower bound of LHS. In addition, if $\mbt_i(X,\cP,D)$ is infeasible, then the recurrence should return $\mbt_i(X,\cP,D)=-\infty$. We will show the upper and lower bound and the infeasible case with a proof by induction depending on the tree node type.

\paragraph{Leaf:} For the base case, i.e. when $i$ is a leaf tree node, the only vertex in $G_i$ is $s'$. The only input for which $\mbt_i(X,\cP,D)$ is feasible is $X=\{s'\},\cP=\set{\set{s'}}$, and $D(s')=0$. For the feasible input, the node $s'$ must be included in the optimal binary forest $F$ otherwise constraint \ref{DP2} will be violated. Since no edges have been introduced in the subtree rooted at tree node $i$, the degree of $s'$ in the optimal binary forest $F$ will be zero. Therefore, $\mbt_i(X,\cP,D) = 0$. If $\mbt_i(X,\cP,D)$ is infeasible, then it is set to $-\infty$.\\

Suppose that $\mbt_j(X,\cP,D)$ is correct for all possible inputs $(X,\cP,D)$ for all children $j$ of a non-leaf tree node $i$. We will show that $\mbt_i(X,\cP,D)$ computed using the recurrence relation based on its children is correct. We consider the various types for tree node $i$.

\paragraph{Introduce vertex:}
Suppose that $i$ has one child $j$ with $X_i = X_j \cup \{v\}$ for some $v \in V(G) \setminus X_j$. We recall that \emph{none} of the edges incident to $v$ have been introduced in the subtree rooted at $i$, so the vertex $v$ is isolated in $G_i$, i.e. $\deg_{G_i}(v)=0$. 
Suppose that $\mbt_i(X,\cP,D)$ is feasible with $F$ being an optimal binary forest. We have two cases:

\emph{Case 1:} Suppose that $v \in X$. Then $\set{v}$ must be a part of $\cP$ and $D(v)=0$ (i.e., condition \ref{IV2} is satisfied), otherwise $\mbt_i(X,\cP,D)$ is infeasible. If \ref{IV2} holds, then $(V(F) \setminus \{v\}, E(F))$ is  a feasible solution for $\mbt_j(X\setminus \{v\},\cP \setminus \{\{v\}\},D')$, where $D':X\setminus \{v\}\rightarrow \{0,1,2,3\}$ is obtained by setting $D'(u)=D(u)$ for every $u\in X\setminus \{v\}$. Hence, $\mbt_i(X,\cP,D) \leq \mbt_j(X \setminus \{v\},\cP \setminus \{\{v\}\},D')$. Since there is a feasible forest $F_j$ for $\mbt_j(X\setminus \{v\},\cP \setminus \{\{v\}\},D')$, a feasible forest for $\mbt_i(X,\cP,D)$ can be obtained by adding an isolated vertex $v$ to $V(F_j)$. Therefore, $\mbt_i(X,\cP,D) \geq \mbt_j(X \setminus \{v\},\cP \setminus \{\{v\}\},D')$.

\emph{Case 2:} Suppose $v \notin X$. Then $v$ is not in $F$. The forest $F$ is a feasible solution for $\mbt_j(X,\cP,D)$. Hence, $\mbt_i(X,\cP,D) \leq \mbt_j(X,\cP,D)$. Since there is a feasible forest $F_j$ for $\mbt_j(X,\cP ,D)$, and $F_j$ is also feasible for $\mbt_i(X,\cP,D)$, we have $\mbt_i(X,\cP,D) \geq \mbt_j(X,\cP,D)$.

Next, suppose that $\mbt_i(X,\cP,D)$ is infeasible. If \ref{IV1} holds, then we are done. Suppose \ref{IV1} fails, but \ref{IV2} holds. In this case, $\mbt_j(X\setminus \{v\},\cP \setminus \{\{v\}\},D')$, where $D':X\setminus \{v\}\rightarrow \{0,1,2,3\}$ is obtained by setting $D'(u)=D(u)$ for every $u\in X\setminus \{v\}$, is infeasible. Hence, $\mbt_i(X,\cP,D)=\mbt_j(X\setminus \{v\},\cP \setminus \{\{v\}\},D')=-\infty$. Suppose that both \ref{IV1} and \ref{IV2} fail. In this case, $\mbt_j(X,\cP,D)$ is infeasible. Hence, $\mbt_i(X,\cP,D)=\mbt_j(X,\cP,D)=-\infty$.

\paragraph{Introduce edge:}
Suppose $i$ introduces edge $\set{u,v}$ and has one child $j$ such that $X_i = X_j$. Suppose that $\mbt_i(X,\cP,D)$ is feasible with $F$ being an optimal binary forest. We have two cases:

\emph{Case 1:} Suppose $u$ and $v$ are both in $X$ and also in the same part of $\cP$ (i.e., condition \ref{IE1} is satisfied). Then, the forest $F$ can either include or exclude $\{u,v\}$.

If $\{u,v\}$ is excluded, then $F$ is also feasible for $\mbt_j(X,\cP,D)$ and hence $\mbt_i(X,\cP,D) \leq \mbt_j(X,\cP,D)$. There is a feasible forest for $\mbt_j(X,\cP ,D)$ which is also feasible for $\mbt_i(X,\cP,D)$. Therefore, $\mbt_i(X,\cP,D) \geq \mbt_j(X,\cP,D)$.

If $\{u,v\}$ is included, then $\cP$ must have a part $P$ that can be partitioned into two disjoint parts $\cP_u$ and $\cP_v$ where $u \in \cP_u$ and $v \in \cP_v$. Hence, the forest $(V(F) \setminus \{u,v\}, E(F) \setminus \{\{u,v\}\})$ is also feasible for $\mbt_j(X,\cP',D')$ for some $\cP' = \cP \setminus \{P\} \cup \{P_u, P_v\}$ with $P=P_u\cup P_v$, and $D':X\rightarrow \{0,1,2,3\}$ obtained by setting $D'(w) = D(w)$ for $w \in X \setminus \set{u,v}$, $D'(u) = D(u)-1$, and $D'(v) = D(v)-1$. Consequently, $\mbt_i(X,\cP,D) \le \maxx_{\cP',D'}{\mbt_j(X,\cP',D')+1}$. On the other hand, a feasible forest for $\mbt_i(X,\cP,D)$ can be obtained by adding edge $\{u,v\}$ to a feasible forest for $\mbt_j(X,\cP',D')$, so $\mbt_i(X,\cP,D) \ge \maxx_{\cP',D'}{\mbt_j(X,\cP',D')+1}$.

\emph{Case 2:} Otherwise, either (1) $u \notin X$ or $v \notin X$, or (2) $u$ and $v$ are both in $X$ but not in the same part of $\cP$. In this case $\{u,v\}$ cannot be in $F$. Hence, the forest $F$ is a feasible solution for the subproblem $\mbt_j(X,\cP,D)$ and hence $\mbt_i(X,\cP,D) \leq \mbt_j(X,\cP,D)$. There is a feasible forest for $\mbt_j(X,\cP ,D)$ which is also feasible for $\mbt_i(X,\cP,D)$. Therefore, $\mbt_i(X,\cP,D) \geq \mbt_j(X,\cP,D)$.

Next, suppose that $\mbt_i(X,\cP,D)$ is infeasible. Then, $\mbt_j(X,\cP,D)$ is also infeasible and hence, $\mbt_j(X,\cP,D)=-\infty$. We consider \ref{IE1} now: In this case, for every partition $\cP' = \cP \setminus \{P\} \cup \{P_u, P_v\}$ with $P=P_u\cup P_v$, and for $D':X\rightarrow \{0,1,2,3\}$ obtained by setting $D'(w) = D(w)$ for $w \in X \setminus \set{u,v}$, $D'(u) = D(u)-1$, and $D'(v) = D(v)-1$, we have that $\mbt_j(X,\cP',D')$ is infeasible. Therefore $\maxx_{\cP',D'}{\mbt_j(X,\cP',D')}=-\infty$.

\paragraph{Drop:}
Suppose $i$ drops $v$ and has a child $j$ such that $X_i = X_j \setminus \{v\}$ for some $v \in X_j$. Suppose that $\mbt_i(X,\cP,D)$ is feasible with $F$ being an optimal binary forest.

If $F$ excludes $v$, then $F$ is also a feasible solution for $\mbt_j(X,\cP,D)$ and hence $\mbt_i(X,\cP,D) \leq \mbt_j(X,\cP,D)$. There is a feasible forest for $\mbt_j(X,\cP ,D)$ which is also feasible for $\mbt_i(X,\cP,D)$. Therefore, $\mbt_i(X,\cP,D) \geq \mbt_j(X,\cP,D)$.

Suppose that $F$ includes $v$, then the forest $F$ is a feasible solution for some $\mbt_j(X \cup \set{v},\cP',D')$, where $\cP'$ is a partition obtained by adding $v$ to one of the existing parts of $\cP$ and $D':X\cup\set{v} \rightarrow \set{0,1,2,3}$ is obtained by setting $D'(u)=D(u)$ for $u \in X$ and $D'(v)$ is set to some value in $\{1,2,3\}$. Hence, $\mbt_i(X,\cP,D)\le \maxx_{\cP',D'}{\mbt_j(X \cup \set{v},\cP',D')}$. On the other hand, a feasible forest for $\mbt_i(X,\cP,D)$ can be obtained by selecting a feasible forest for $\mbt_j(X,\cP',D')$, so $\mbt_i(X,\cP,D) \ge \maxx_{\cP',D'}{\mbt_j(X \cup \set{v},\cP',D')}$.

Next, suppose that $\mbt_i(X,\cP,D)$ is infeasible. Then, $\mbt_j(X,\cP,D)$ is also infeasible and hence $\mbt_j(X,\cP,D)=-\infty$. Moreover, for every partition $\cP'$ obtained by adding $v$ to one of the existing parts of $\cP$ and every $D':X\cup\set{v} \rightarrow \set{0,1,2,3}$ obtained by setting $D'(u)=D(u)$ for $u \in X$ and every choice of $D'(v)\in \{1,2,3\}$, there is no feasible forest for $\mbt_j(X\cup \set{v},\cP',D')$. Hence, $\maxx_{\cP',D'}{\mbt_j(X \cup \set{v},\cP',D')}=-\infty$.

\paragraph{Join:}
Suppose $i$ has two children $j$ and $k$ and $X_i=X_j=X_k$. Suppose that $\mbt_i(X,\cP,D)$ is feasible with $F$ being an optimal binary forest.

First we show that LHS $\leq$ RHS. By Lemma~\ref{lem:disjoint}, the edges in $F$ are from disjoint edge sets $E_j$ and $E_k$. Hence, the forest $F$ decomposes into two binary forests $F_j:=(V(F) \cap V_j ,E(F)\cap E_j)$ and $F_k:=(V(F) \cap V_k ,E(F)\cap E_k)$. In particular $F_j$ and $F_k$ are subgraphs of $G_j$ and $G_k$, respectively. Let $X^j := V(F_j) \cap X_j$ be the set of vertices in $X_j$ that belong to $F_j$ and similarly, let $X^k:=V(F_k)\cap X_k$.

\begin{claim} \label{cl:sameX}
$X^j = X^k = X$.
\end{claim}
\begin{proof}
We will show that $X^j=X$. The proof for $X^k=X$ will also follow by the same argument. 

We first have that $X \subseteq X^j$ because $X \subseteq V(F)$ and $X \subseteq X_i = X_j \subseteq V_j$ imply $X \subseteq V(F) \cap V_j \cap X_j = X^j$. Next, suppose that there exists a vertex $v \in X^j \setminus X$. Then $v \in X_j \setminus X = X_i \setminus X$. Besides, $v \in V(F_j) \subseteq V(F)$. However, these two statements violate \ref{DP3} so $X^j \subseteq X$.
\end{proof}

We show that there exist partitions $\cP^j$ and $\cP^k$ of $X$, degree requirements $D^j$, $D^k: X\rightarrow \{0,1,2,3\}$, and a decomposition of the forest $F$ into $F^j$ and $F^k$ such that
\begin{enumerate} [label=(J\arabic*)]
\item \label{J2} the merged graph $H(\cP^j,\cP^k)$ is a forest,
\item \label{J3} the partition $\mathcal{Q}(\cP^j,\cP^k)$ is exactly $\cP$,
\item \label{J4} $D^j(v) + D^k(v) = D(v)$ for $v \in X$, and
\item \label{J1} $F_j$ is feasible for $\mbt_j(X,\cP^j,D^j)$ and $F_k$ is feasible for $\mbt_k(X,\cP^k,D^k)$.
\end{enumerate}

Let $b \in \{j,k\}$. We obtain the partition $\cP^b$ of $X$ as follows: vertices of $X$ in the same connected component of $F_b$ will be in the same part of $\cP^b$, i.e., if $\mathcal{R}'_b$ is a partition of $V(F_b)$ based on the connected components of $F_b$, then $\cP^b=\{R'\cap X| R'\in \mathcal{R}_b'\}$.

We recall that $H_b$ is an auxiliary graph that contains vertices for every vertex in $X$ and vertices for every part in $\cP^b$, with the vertex corresponding to a part of $\cP^b$ being adjacent to all vertices that are in that part. The merged graph $H(\cP^j,\cP^k) := (V(H_j) \cup V(H_k), E(H_j) \cup E(H_k))$ where $V(H_j)\cap V(H_k)=X$ is such that $E(H_j)\cap E(H_k)=\emptyset$. Let $u, v \in X$. For brevity, we denote \emph{$u$-$v$ path} as a path between $u$ and $v$. From the fact that (1) $u$ and $v$ are in the same part of $\cP^j$ (or $\cP^k$) if and only if their is a unique $u$-$v$ path in $F_j$ (or $F_k$) and (2) $u$ and $v$ are in the same part of $\cP^j$ (or $\cP^k$) if and only if their is a unique $u$-$v$ path in $H_j$ (or $H_k$), we have the following observation:

\begin{observation}\label{obs:path}
Let $u, v \in X$, then there is a unique $u$-$v$ path in $F_j$ (or $F_k$) if and only there is a unique $u$-$v$ path in $H_j$ (or $H_k$).
\end{observation}

\begin{claim}
The merged graph $H(\cP^j,\cP^k)$ satisfies \ref{J2}. 
\end{claim}
\begin{proof}
The proof consists of showing two parts: (1) if $u, v \in X$ and there is a $u$-$v$ path in $H(\cP^j,\cP^k)$, then this path is unique, and (2) there is no cycle in $H(\cP^j,\cP^k)$. We will use the notation $u - F_j - v$ to denote that there is a unique $u$-$v$ path in $F_j$ and such a path may have intermediary vertices from $X \setminus \{u,v\}$. We will use similar notations for $F_k$, $H_j$, and $H_k$.

Let $u, v \in X$. Suppose that there is a $u$-$v$ path in $H(\cP^j,\cP^k)$. Since $E(H_j) \cap E(H_k) = \emptyset$ and $(V(H_j) \setminus X) \cap (V(H_k) \setminus X) = \emptyset$, the path must be one of the following:
\begin{enumerate}
\item $u - H_j - w_1 - H_k - w_2 - ... - w_{n-1} - H_k - w_n - H_j - v$,
\item $u - H_j - w_1 - H_k - w_2 - ... - w_{n-1} - H_j - w_n - H_k - v$,
\item $u - H_k - w_1 - H_j - w_2 - ... - w_{n-1} - H_k - w_n - H_j - v$, or
\item $u - H_k - w_1 - H_j - w_2 - ... - w_{n-1} - H_j - w_n - H_k - v$
\end{enumerate}
where $w_1, ..., w_n \in X \setminus \{u,v\}$. In short, a $u$-$v$ path in $H(\cP^j,\cP^k)$ must alternate edges between $H_j$ and $H_k$. By Observation~\ref{obs:path}, if the $u$-$v$ path in $H(\cP^j,\cP^k)$ is the first case, then there is a $u$-$v$ path $u - F_j - w_1 - F_k - w_2 - ... - w_{n-1} - F_k - w_n - F_j - v$ in $F$. The argument is similar for the other three cases. We note that the mapping of a $u$-$v$ path in $H(\cP^j,\cP^k)$ to a $u$-$v$ path in $F$ is a bijection. If there are two $u$-$v$ paths in $H(\cP^j,\cP^k)$, then there are two $u$-$v$ paths in $F$ and $F$ is not a forest, a contradiction. Therefore, we have the following observation:

\begin{observation} \label{obs:bij}
Let $u, v \in X$. There is no $u$-$v$ path in $F$ if and only if there is no $u$-$v$ path in $H(\cP^j,\cP^k)$. If there is a $u$-$v$ path in $F$, then there is a bijection between the unique $u$-$v$ path in $F$ and the unique $u$-$v$ path in $H(\cP^j,\cP^k)$.
\end{observation}

This implies that if $u, v \in X$ and there is a $u$-$v$ path in $H(\cP^j,\cP^k)$, then this path is unique.
Next, suppose that there is a cycle in $H(\cP^j,\cP^k)$. Then this cycle has even length in $H(\cP^j,\cP^k)$ since $H(\cP^j,\cP^k)$ is bipartite with $X$ on one side and vertices for every part in $\cP^j$ or $\cP^k$ on the other side. Furthermore, the cycle has length at least four and alternates vertices from $X$ and from parts in $\cP^j$ or $\cP^k$. This indicates that there must be two vertices $u,v \in X$ in the cycle, which contradicts the fact that if there is a $u$-$v$ path in $H(\cP^j,\cP^k)$, then such a path must be unique.
\end{proof}

\begin{claim}
The partition $\mathcal{Q}(\cP^j, \cP^k)$ satisfies \ref{J3}.
\end{claim}
\begin{proof}
Let $\mathcal{Q'}$ be a partition of $V(H(\cP^j,\cP^k))$ where vertices in the same connected component of $H(\cP^j,\cP^k)$ belong to the same part of $\mathcal{Q'}$. We recall that $\mathcal{Q}(\cP^j, \cP^k)$ is the partition of $X$ obtained from $\mathcal{Q}'$ by restricting each part of $\mathcal{Q}'$ to elements in $X$. That is, $\mathcal{Q}(\cP^j, \cP^k) = \{Q \cap X \mid Q \in \mathcal{Q'} \}$.

We prove \ref{J3} by showing that the following statements are equivalent for $u,v \in X$: 
\begin{enumerate} [label=(P\arabic*)]
\item \label{P1} $u$ and $v$ are in the same part of $\cP$,
\item \label{P2} there is a unique $u$-$v$ path in $F$,
\item \label{P3} there is a unique $u$-$v$ path in $H(\cP^j,\cP^k)$, and
\item \label{P4} $u$ and $v$ are in the same part of $\mathcal{Q}(\cP^j,\cP^k)$.
\end{enumerate}

\ref{P1}$\iff$\ref{P2}: This is by the definition of $\cP$. The vertices $u$ and $v$ are in the same part of $\cP$ if and only if they are in the same connected component of $F$. Since $F$ is a forest, the vertices $u$ and $v$ are in the same connected component of $F$ if and only if there is a unique $u$-$v$ path in $F$.

\ref{P2}$\iff$\ref{P3}: This is by Observation~\ref{obs:bij}.

\ref{P3}$\iff$\ref{P4}: Since $H(\cP^j,\cP^k)$ is a forest, there is a unique $u$-$v$ path in $H(\cP^j,\cP^k)$ if and only if $u$ and $v$ are in the same connected component of $H(\cP^j,\cP^k)$. By the definition of $\mathcal{Q}(\cP^j,\cP^k)$, $u$ and $v$ are in the same connected component of $H(\cP^j,\cP^k)$ if and only if they are in the same part of $\mathcal{Q}(\cP^j,\cP^k)$.

From \ref{P1}$\iff$\ref{P4}, we know that $\mathcal{Q}(\cP^j,\cP^k) = \cP$.
\end{proof}

For \ref{J4}, we set $D^j(v) := \deg_{F_j}(v)$ and $D^k(v) := \deg_{F_k}(v)$ for $v \in X$. By the edge disjointness of $F_j$ and $F_k$, we have $D^j(v) + D^k(v) = \deg_{F_j}(v) + \deg_{F_k}(v) = \deg_F(v) = D(v)$.

Now we show \ref{J1}.

\begin{claim}
$F_j$ is feasible for $\mbt_j(X,\cP^j,D^j)$ and $F_k$ is feasible for $\mbt_k(X,\cP^k,D^k)$.
\end{claim}
\begin{proof}
We will show that $F_j$ is feasible for $\mbt_j(X,\cP^j,D^j)$. The proof for $F_k$ being feasible for $\mbt_k(X,\cP^k,D^k)$ would follow by the same argument.

We need to show that properties \ref{DP1}, \ref{DP2}, \ref{DP3}, \ref{DP4}, and \ref{DP5} hold. \ref{DP1} holds because $F_j:=(V(F) \cap V_j ,E(F)\cap E_j)$ is a subgraph of $G_j$. \ref{DP2} holds since $s' \in X = X^j$ where $X^j := V(F_j) \cap X_j$. This is obtained from the fact that $F$ is feasible for $\mbt_i(X,\cP,D)$, which implies $s' \in X$, and $X^j = X$ by Claim~\ref{cl:sameX}. \ref{DP3} holds because of Claim~\ref{cl:sameX}. \ref{DP4} holds by the definition of $\cP^j$: vertices of $X$ in the same connected component of $F_j$ will be in the same part of $\cP^j$. \ref{DP5} holds by the definition $D^j(v) := \deg_{F_j}(v)$ for every $v \in X$.
\end{proof}

We have shown that there exist partitions $\cP^j$, $\cP^k$ of $X$, degree requirements $D^j, D^k: X\rightarrow \{0,1,2,3\}$, and a decomposition of the forest $F$ into $F^j$ and $F^k$ such that \ref{J2}, \ref{J3}, \ref{J4}, and \ref{J1} hold. Therefore, $\mbt_i(X,\cP,D) \leq \maxx_{\cP^j,\cP^k,D^j,D^k}{\mbt_j(X,\cP^j,D^j)+\mbt_k(X,\cP^k,D^k)}$.\\

Next, we show that LHS $\geq$ RHS. Given input $(X,\cP,D)$ at tree node $i$, suppose that we have partitions $\cP^j$ and $\cP^k$ of $X$, and degree requirements $D^j, D^k: X\rightarrow \{0,1,2,3\}$ such that
\begin{enumerate}
\item the merged graph $H(\cP^j,\cP^k)$ is a forest,
\item the partition $\mathcal{Q}(\cP^j,\cP^k)$ is exactly $\cP$,
\item $D^j(v) + D^k(v) = D(v)$ for $v \in X$, and
\item there are feasible forests $F_j$ for $\mbt_j(X,\cP^j,D^j)$ and $F_k$ for $\mbt_k(X,\cP^k,D^k)$. 
\end{enumerate}

We show that $F':=(V(F_j) \cup V(F_k), E(F_j) \cup E(F_k))$ is a feasible forest for $\mbt_i(X,\cP,D)$ with $\mbt_j(X,\cP^j,D^j) + \mbt_k(X,\cP^k,D^k)$ edges. This consists of showing the following: (1) $|E(F')| = \mbt_j(X,\cP^j,D^j) + \mbt_k(X,\cP^k,D^k)$, (2) $F'$ is a forest, and (3) $F'$ is feasible for $\mbt_i(X,\cP,D)$.

For the first part, we note that $F_j$ and $F_k$ are subgraphs of $G_j$ and $G_k$, respectively. By Lemma~\ref{lem:disjoint}, we have $E(G_j) \cap E(G_k) = \emptyset$ which implies $E(F_j) \cap E(F_k) = \emptyset$ and $|E(F')| = |E(F_j)| + |E(F_k)| = \mbt_j(X,\cP^j,D^j) + \mbt_k(X,\cP^k,D^k)$.

We now prove that $F'$ is a forest. Similar to the argument while proving LHS $\leq$ RHS, we note that Observation~\ref{obs:path} still holds.

\begin{claim}
$F'$ is a forest.
\end{claim}
\begin{proof}
The proof consists of showing two parts: (1) if $u, v \in X$ and there is a $u$-$v$ path in $F'$, then this path is unique, and (2) there is no cycle in $F'$.

Let $u,v \in X$. Since $E(F_j) \cap E(F_k) = \emptyset$ and $(V(F_j) \setminus X_i) \cap (V(F_k) \setminus X_i) = \emptyset$, if there is a $u$-$v$ path in $F'$, it must be one of the following:
\begin{enumerate}
\item $u - F_j - w_1 - F_k - w_2 - ... - w_{n-1} - F_k - w_n - F_j - v$,
\item $u - F_j - w_1 - F_k - w_2 - ... - w_{n-1} - F_j - w_n - F_k - v$,
\item $u - F_k - w_1 - F_j - w_2 - ... - w_{n-1} - F_k - w_n - F_j - v$, or
\item $u - F_k - w_1 - F_j - w_2 - ... - w_{n-1} - F_j - w_n - F_k - v$
\end{enumerate}
where $w_1, ..., w_n \in X \setminus \{u,v\}$. By Observation~\ref{obs:path}, if the $u$-$v$ path in $F'$ is the first case, then there is a $u$-$v$ path $u - H_j - w_1 - H_k - w_2 - ... - w_{n-1} - H_k - w_n - H_j - v$ in $H(\cP^j,\cP^k)$. The argument is similar for the other three cases. We note that the mapping of a $u$-$v$ path in $F'$ to a $u$-$v$ path in $H(\cP^j,\cP^k)$ is a bijection. If there are two $u$-$v$ paths in $F'$, then there are two $u$-$v$ paths in $H(\cP^j,\cP^k)$ and $H(\cP^j,\cP^k)$ is not a forest, a contradiction. Therefore, we have the following observation:

\begin{observation} \label{obs:bij2}
Let $u, v \in X$. There is no $u$-$v$ path in $H(\cP^j,\cP^k)$ if and only if there is no $u$-$v$ path in $F'$. If there is a $u$-$v$ path in $H(\cP^j,\cP^k)$, then there is a bijection between the unique $u$-$v$ path in $H(\cP^j,\cP^k)$ and the unique $u$-$v$ path in $F'$.
\end{observation}

This implies that if $u, v \in X$ and there is a $u$-$v$ path in $F'$, then this path is unique. Now, if $F'$ has a cycle, then this cycle must have two vertices $u,v \in X$ because $(V(F_j) \setminus X_i) \cap (V(F_k) \setminus X_i) = \emptyset$. This implies that there are two $u$-$v$ paths in $F'$, a contradiction.
\end{proof}

Finally, we show that $F'$ is feasible for $\mbt_i(X,\cP,D)$.

\begin{claim}
The forest $F'$ is feasible for $\mbt_i(X,\cP,D)$.
\end{claim}
\begin{proof}
We need to show \ref{DP1}, \ref{DP2}, \ref{DP3}, \ref{DP4}, and \ref{DP5}. \ref{DP1} holds because $F':=(V(F_j) \cup V(F_k), E(F_j) \cup E(F_k))$ is a subgraph of $G_i = (V(G_j) \cup V(G_k), E(G_j) \cup E(G_k))$. \ref{DP2} holds because we know $s' \in X$ from the feasibility of $\mbt_j(X,\cP^j,D^j)$ (or $\mbt_k(X,\cP^k,D^k)$). \ref{DP3} holds because $X_i = X_j = X_k$ and $X = X_i \cap V(F')$. To show $X = X_i \cap V(F')$, first $X = X_j \cap V(F_j) \subseteq X_i \cap V(F')$ and $X_i \cap V(F') = X_i \cap (V(F_j) \cup V(F_k)) = X_i \cap (X \cup (V(F_j) \setminus X) \cup (V(F_k) \setminus X)) = X_i \cap X \subseteq X$. \ref{DP5} holds by edge disjointness of $F_j$ and $F_k$ and the fact that $D(v) = D^j(v) + D^k(v)$ for every $v \in X$.

Now we prove \ref{DP4}, namely for $u,v \in X$, if $u$ and $v$ are in the same connected component of $F'$, then $u$ and $v$ are in the same part of $\cP$. We show that the following statements are equivalent for $u,v \in X$,
\begin{enumerate} [label=(P\arabic*$'$)]
\item \label{P1'} $u$ and $v$ are in the same connected component of $F'$,
\item \label{P2'} there is a unique $u$-$v$ path in $F'$,
\item \label{P3'} there is a unique $u$-$v$ path in $H(\cP^j,\cP^k)$, and
\item \label{P4'} $u$ and $v$ are in the same part of $\mathcal{Q}(\cP^j,\cP^k) = \cP$.
\end{enumerate}

\ref{P1'} $\iff$ \ref{P2'}: Since $F'$ is a forest, $u$ and $v$ are in the same connected component of $F'$ if and only if there is a unique $u$-$v$ path in $F'$.

\ref{P2'} $\iff$ \ref{P3'}: This is by Observation~\ref{obs:bij2}.

\ref{P3'} $\iff$ \ref{P4'}: This is by the definition of $\mathcal{Q}(\cP^j,\cP^k)$. Vertices $u$ and $v$ are in the same connected component of $H(\cP^j,\cP^k)$ if and only if they are in the same part of $\mathcal{Q}(\cP^j,\cP^k)$. Since $H(\cP^j,\cP^k)$ is a forest, there is a unique $u$-$v$ path in $H(\cP^j,\cP^k)$ if and only if $u$ and $v$ are in the same part of $\mathcal{Q}(\cP^j,\cP^k)$.
\end{proof}

Since $F'$ is a feasible forest with $\mbt_j(X,\cP^j,D^j) + \mbt_k(X,\cP^k,D^k)$ edges for $\mbt_i(X,\cP,D)$, we have $\mbt_i(X,\cP,D) \geq \maxx_{\cP^j,\cP^k,D^j,D^k}{\mbt_j(X,\cP^j,D^j)+\mbt_k(X,\cP^k,D^k)}$.

Next, suppose that $\mbt_i(X,\cP,D)$ is infeasible. For every $\cP^j$ and $\cP^k$ such that $H(\cP^j,\cP^k)$ is a forest, $\mathcal{Q}(\cP^j,\cP^k) = \cP$ is the resulting partition on $X$, and for every $D^j,D^k:X\rightarrow \{0,1,2,3\}$ such that $D(v) = D^j(v) + D^k(v)$ for every $v \in X$, either $\mbt_j(X,\cP^j,D^j)=-\infty$ or $\mbt_k(X,\cP^k,D^k)=-\infty$, otherwise we can find a feasible solution and this contradicts the assumption that $\mbt_i(X,\cP,D)$ is infeasible. If such $\cP^j,\cP^k,D^j$, and $D^k$ do not exist, then $\mbt_i(X,\cP,D)=-\infty$.
\end{proof}

==> relatedwork.tex <==
\subsection{Related work}
Degree-constrained subgraph problems appeared as early as 1978 in the textbook of Garey and Johnson \cite{GJ-book} and have garnered plenty of attention in the approximation community  \cite{Gab83,EFRS90,FR94,RMRRH01,ADR08, KKN08, LNSS09, SL15}. A rich line of works have addressed the minimum degree spanning tree problem as well as the minimum cost degree-constrained spanning tree problem leading to powerful rounding techniques and a deep understanding of the spanning tree polytope \cite{CRRT09a,CRRT09b,KR02, KR05,Goe06,SL15,FR94}. Approximation and bicriteria approximation algorithms for the counterparts of these problems in directed graphs, namely degree-constrained arborescence and min-cost degree-constrained arborescence, have also been studied in the literature \cite{BKN09}. 

In the \emph{maximum-edge} degree-constrained connected subgraph problem, the goal is to find a connected degree-constrained subgraph of a given graph with maximum number of edges. This problem does not admit a PTAS \cite{APPSS09} and has been studied from the perspective of fixed-parameter tractability \cite{ASS08}. 
MBT could be viewed as a \emph{maximum-vertex} degree-constrained connected subgraph problem, where the goal is to maximize the number of \emph{vertices} as opposed to the number of \emph{edges}---the degree-constrained connected subgraph maximizing the number of vertices may be assumed to be acyclic and hence, a tree. 
It is believed that the \emph{connectivity constraint} makes the maximum-edge degree-constrained connected subgraph problem to become extremely difficult to approximate. Our results formalize this belief when the objective is to maximize the number of vertices. 

Switching the objective with the constraint in the maximum-vertex degree-constrained connected subgraph problem leads to the minimum-degree $k$-tree problem: here the goal is to find a minimum degree subgraph that is a tree with at least $k$ vertices. Minimum degree $k$-tree admits a $O(\sqrt{(k/\Delta^*)\log{k}})$-approximation, where $\Delta^*$ is the optimal degree and does not admit a $o(\log{n})$-approximation \cite{KKN08}. We note that the hardness reduction here (from set cover) crucially requires the optimal solution value $\Delta^*$ to grow with the number $n$ of vertices in the input instance, and hence, does not imply any hardness result for input instances in which $\Delta^*$ is a constant. Moreover, the approximation result implies that a tree of degree $O(\sqrt{k\log{k}})$ containing $k$ vertices can be found in polynomial time if the input graph contains a constant-degree tree with $k$ vertices.

We consider the maximum binary tree problem to be a generalization of the longest path problem as both can be viewed as asking for a maximum-sized degree-constrained connected acyclic subgraph. The longest path problem in undirected graphs admits an $\Omega\tp{{(\log{n}/\log\log{n})^2}/{n}}$-approximation \cite{BHK04}, but it is APX-hard and does not admit a $2^{-O\tp{\log^{1-\eps}{n}}}$-approximation for any constant $\eps>0$ unless $\NP \subseteq \DTIME{2^{\log^{O(1/\eps)}{n}}}$ \cite{karger1997approximating}. Our hardness results for the max binary tree problem in undirected graphs bolsters this connection. The longest path problem in directed graphs is much harder: For every $\eps >0$ it cannot be approximated to within a factor of $1/n^{1-\eps}$ unless $\P = \NP$, and it cannot be approximated to within a factor of $(\log^{2+\eps} n)/n$ under the Exponential Time Hypothesis \cite{BHK04}. However, the longest path problem in DAGs is solvable in polynomial time. Our hardness results for the max binary tree problem in DAGs are in stark contrast to the polynomial-time solvability of the longest path problem in DAGs. 

On the algorithmic side, the color-coding technique introduced by Alon, Yuster, and Zwick \cite{alon1995color} can be used to decide whether an undirected graph $G=(V,E)$ contains a copy of a bounded treewidth pattern graph $H=(V_H, E_H)$ where $|V_H|=O\tp{\log|V|}$, and if so, then find one in polynomial time. The idea here is to randomly color the vertices of $G$ by $O\tp{\log|V|}$ colors and to find a maximum colorful copy of $H$ using dynamic programming. The same dynamic programming approach can be modified to find a maximum colorful binary tree. This algorithm can be derandomized, thus leading to a deterministic $\Omega\tp{({1}/{n})\log{n}}$-approximation to \umaxBT. 

In parameterized complexity, designing algorithms with running time $\beta^k \poly(n)$ ($\beta > 1$ is a constant) for problems like \kpath and $k$-\textsc{Tree} is a central topic.  For \kpath, the color-coding technique mentioned above already implies a $(2e)^k \poly(n)$-time algorithm. Koutis \cite{koutis2008faster} noticed that \kpath can be reduced to detecting whether a given polynomial contains a multilinear term. Using algebraic methods for the latter problem, Koutis obtained a $2^{1.5k} \poly(n)$ time algorithm for \kpath. This was later improved by Williams \cite{williams2009finding} to $2^k \poly(n)$. The current state-of-art algorithm is due to Bj\"orklund, Husfeldt, Kaski and Koivisto 
\cite{bjorklund2017narrow}, which is also an algebraic algorithm with running time $1.66^k \poly(n)$.
All of these algorithms are randomized. 
Our study of the \kBT problem, which is the problem of deciding whether a given graph $G$ contains a binary tree of size at least $k$, is inspired by this line of results. 
%Inspired by these results, we study the same problem for \kBT, which is the problem of deciding whether a given graph $G$ contains a binary tree of size at least $k$.

\iffalse
Several $\NP$-hard problems are known to be solvable in specific families of graphs. Bipartite permutation graphs and bounded treewidth graphs are two such families which are known to exhibit this behaviour \cite{FPT-book,Efficient_Alg_Longest_Path,smith2011minimum,spinrad1987bipartite,KLOKS1998313}. Our polynomial-time solvability result for these families of graphs crucially identifies the existence of structured optimal solutions to reduce the search space and solves the problem over this reduced search space.
\fi

Several $\NP$-hard problems are known to be solvable in specific families of graphs. Bipartite permutation graphs 
%and bounded treewidth graphs are two such families which are 
is one such family which is 
known to exhibit this behaviour %\cite{FPT-book,Efficient_Alg_Longest_Path,smith2011minimum,spinrad1987bipartite,KLOKS1998313}. 
\cite{Efficient_Alg_Longest_Path, smith2011minimum,spinrad1987bipartite,KLOKS1998313}.
Our polynomial-time solvability result for this family of graphs crucially identifies the existence of structured optimal solutions to reduce the search space and solves the problem over this reduced search space.

\subsection{Organization} We start with preliminary definitions in Section \ref{sec:prelim}. We present our hardness results for DAGs in Section \ref{sec:hardness-dags}. We show a  natural  IP for DAGs and its integrality gap in Section \ref{sec:integrality-gap}. We show our hardness results for undirected graphs in Section \ref{sec:undirected-hardness}. We present a $2^k \poly(n)$ time algorithm for \kBT in Section \ref{sec:arithmetization}. We design an efficient algorithm for bipartite permutation graphs in Section \ref{sec:bipartite-permutation}. 
%We present an efficient algorithm for finding a maximum binary tree in bounded treewidth graphs in Section \ref{sec:boundedtreewidth}. 
We conclude with a few open problems in Section \ref{sec:conclusions}.
